Finding many Collisions via Reusable Quantum Walks

Given a random function $f$ with domain $[2^n]$ and codomain $[2^m]$, with $m \geq n$, a collision of $f$ is a pair of distinct inputs with the same image. Collision finding is an ubiquitous problem in cryptanalysis, and it has been well studied using both classical and quantum algorithms. Indeed, the quantum query complexity of the problem is well known to be $\Theta(2^{m/3})$, and matching algorithms are known for any value of $m$. The situation becomes different when one is looking for multiple collision pairs. Here, for $2^k$ collisions, a query lower bound of $\Theta(2^{(2k+m)/3})$ was shown by Liu and Zhandry (EUROCRYPT~2019). A matching algorithm is known, but only for relatively small values of $m$, when many collisions exist. In this paper, we improve the algorithms for this problem and, in particular, extend the range of admissible parameters where the lower bound is met. Our new method relies on a chained quantum walk algorithm, which might be of independent interest. It allows to extract multiple solutions of an MNRS-style quantum walk, without having to recompute it entirely: after finding and outputting a solution, the current state is reused as the initial state of another walk. As an application, we improve the quantum sieving algorithms for the shortest vector problem (SVP), with a complexity of $2^{0.2563d + o(d)}$ instead of the previous $2^{0.2570d + o(d)}$.

==> files/heuristic-v1.tex <==
% !TeX root = ../collision-walk.tex

\newcommand{\cc}{\mathcal{C}}
\newcommand{\wU}{\widetilde{U}}
\newcommand{\eps}{\varepsilon}
\newcommand{\hh}{\mathcal{H}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\xh}{\widehat{x}}
\newcommand{\yh}{\widehat{y}}
\newcommand{\pxh}{\widehat{p_x}}
\newcommand{\pyh}{\widehat{p_y}}
\newcommand{\SWUP}{\textrm{SWUP}}
\newcommand{\Swap}{\textrm{Swap}}
\newcommand{\UP}{\textrm{UP}}
\newcommand{\Enc}{\textrm{Enc}}
\newcommand{\COMMENT}[1]{}


\section{Heuristic-free Quantum Walks}

We consider a quantum walk with an \emph{imperfect} implementation of the update and setup unitaries (typically, in the subset-sum case). We also consider here that this walk solves a \emph{subset finding} problem as studied in~\cite{DBLP:journals/qic/ChildsE05}:

\begin{problem}[$R$-subset finding]
Given a set of size $X$ with superposition query access, given a relation $R$ of arity $r$, return the tuple $x_1, \ldots, x_r \in X^r$ (a single solution expected, or none) such that $R(x_1, \ldots, x_r)$.
\end{problem}

We will flesh out the precise notion of \emph{imperfect} and the assumptions that we need for the walk to still work. 

%Although subset-sums are our main target, this result can be applied in the context of quantum decoding algorithms~\cite{DBLP:conf/pqcrypto/KachigarT17}, $k$-list and merging algorithms \AS{cite something}. The proof that we give borrow some elements from~\cite{DBLP:journals/siamcomp/Ambainis07,mnrs11,DBLP:journals/qic/ChildsE05,DBLP:journals/siamcomp/BennettBBV97,DBLP:conf/soda/JefferyKM13}.
%
%We assume that the reader is familiar with the basics of quantum computing. A \emph{reflection through} a state $\ket{x}$ is a unitary operator $U$ that applies: $U \ket{x} = \ket{x}$ and $U \ket{y} = - \ket{y}$ if $\ket{y}$ is orthogonal to $\ket{x}$. 

\begin{assumption}[Walk setting]
We are looking for a single solution of an $R$-subset finding problem, using an MNRS quantum walk on a product Johnson graph.
\end{assumption}


\subsection{Perfect Run of the Walk}

We will first consider the MNRS walk with a ``perfect'' update unitary $U$. We will also assume that the setup unitary, which produces the starting state of the walk, is also perfect: it produces the uniform superposition over all vertices of the product Johnson graph.. The walk then applies $\frac{1}{\sqrt{\epsilon}}$ steps. Each step consists in the product of two operators, similarly to Grover's algorithm:
\begin{itemize}
\item an operator which emulates a reflection through the stationary distribution state $\ket{\pi}$
\item an operator which reflects through the uniform superposition of marked vertices $\ket{\mu}$: this is the checking step, which remains exact for us.
\end{itemize}

\paragraph{Basis States in the walk.}
The state of an MNRS walk has three registers ``R'' (right), ``L'' (left) and ``D'' (data structure). We write the basis vectors as $\ket{x}_L \ket{y}_R \ket{\mathcal{D}(x)}_D$ where $(x,y)$ is an edge in the product Johnson graph and $D(x)$ is the data structure that helps determining if $x$ is marked or not. To each state $x \in \Omega$ corresponds a unique data structure $\mathcal{D}(x)$. We define two update unitaries $U_P$ and $U_D$: $U_P$ acts only on the L and R registers, and on input $\ket{x} \ket{0}$, writes the uniform superposition of neighbors. $U_D$ is responsible for updating the data structure. It does:
$$U_D~: \ket{x}_L \ket{y}_R \ket{\mathcal{D}(x)}_D \mapsto \ket{x}_L \ket{y}_R \ket{\mathcal{D}(y)}_D \enspace.$$
Thus $U_D$ transforms $\mathcal{D}(x)$ into the neighboring $\mathcal{D}(y)$. During the course of the quantum walk, the state remains a superposition of basis states $\ket{x} \ket{y} \ket{\mathcal{D}(x)}$ or $\ket{x} \ket{y} \ket{\mathcal{D}(y)}$. 


\begin{lemma}[From~\cite{DBLP:journals/siamcomp/MagniezNRS11}]\label{lemma:walk-tmp}
A step of the walk emulates a product of two reflections through $\ket{\pi}$ and $\ket{\mu}$ in the two-dimensional space spanned by $\ket{\pi}$ and $\ket{\mu}$: $ \mathrm{ref}(\ket{\pi}) \cdot  \mathrm{ref}(\ket{\mu^\bot}) $ where $\ket{\mu^\bot}$ is the state orthogonal to $\ket{\mu}$ forming an acute angle with $\ket{\pi}$. If $\ket{\psi_i}$ is the state after $i$ steps of the walk, the difference
$$\| \ket{\psi_i} -  \left(\mathrm{ref}(\ket{\pi}) \cdot \mathrm{ref}(\ket{\mu^\bot}) \right)^i \ket{\pi} \|  $$
is negligible.
\end{lemma}

\AS{by how much?}

We define the \emph{perfect walk states} $\ket{\phi_i}$ as those obtained using this product of reflections: $\ket{\phi_i} = \left(\mathrm{ref}(\ket{\pi}) \cdot \mathrm{ref}(\ket{\mu^\bot}) \right)^i \ket{\pi}$. For now, we will reason with $\ket{\phi_i}$ only, we will use later the fact that $\| \ket{\psi_i} - \ket{\phi_i}\|$ is negligible (note that it can be made arbitrarily small). In particular, $\ket{\phi_i}$ belongs to a two-dimensional space spanned by the uniform superposition of states  $\ket{x} \ket{y} \ket{\mathcal{D}(x)}$ where $x$ is marked, on one hand, and the uniform superposition of such states where $x$ is not marked, on the other hand. So marked and unmarked vertices have the same amplitudes respectively in $\ket{\phi_i}$. This remains true after $\mathrm{ref}(\ket{\mu^\bot})$, since this unitary simply dephases the amplitudes of marked states.

\begin{lemma}\label{lemma:equalampl}
In $\ket{\phi_i}$, and in $\mathrm{ref}(\ket{\mu^\bot}) \ket{\phi_i}$,  all basis states $\ket{x} \ket{y} \ket{\mathcal{D}(x)}$ where $x$ is marked have the same amplitude. All basis states where $x$ is unmarked also have the same amplitudes.
\end{lemma}


The reflection through $\ket{\pi}$ is obtained in a more efficient way than recomputing the setup (which is what we do in a standard quantum search). This is done via a \emph{phase estimation circuit} for the update step (see Theorems 5 and 6 in~\cite{DBLP:journals/siamcomp/MagniezNRS11}). Reusing the notations of~\cite{DBLP:journals/siamcomp/MagniezNRS11}, we define an operator $W(P)$ that performs a single update step of the Markov chain $P$. In full generality, $W(P)$ first reflects through $\mathrm{span}(\ket{x} \ket{p_x})$, then through $\mathrm{span}(\ket{p_y^*} \ket{y})$. %Since we consider the specific case of a Johnson graph, this transformation can be described explicitly: this is done in~\cite[Algorithm 1]{DBLP:journals/siamcomp/Ambainis07}.

%The update step is divided into two unitaries: $U_P$ and $U_D$, where $U_P$ updates the vertex $x$, and $U_D$ is responsible for updating the data structure $D(x)$. 
In the update step, we will always assume that $U_P$ is exact. Our problem will stem from $U_D$. For now, we look at the walk when $U_D$ is exact.



\paragraph{The phase Estimation Circuit.}
The most technical step is arguably the phase estimation circuit that emulates a reflection through $\ket{\pi}$, using  $\bigOt{\frac{1}{\sqrt{\delta}}}$ calls to $U_D U_P$. For this, we write the current state of the walk as a linear combination of eigenvectors of $U_D U_P$: $ \ket{\psi} = \sum_j \alpha_j \ket{\psi_j} \enspace. $
Each of these eigenvectors is related to an eigenvalue of the form $e^{\pm 2 i \theta_j}$, such that $U_D U_P \ket{\psi_j} = e^{\pm 2 i \theta_j} \ket{\psi_j}$. By properties of the walk, there is a single eigenvector for the eigenvalue $1$ (thus an angle $0$), which is the stationary state $\ket{\pi}$. All other angles are between $\bigO{\frac{1}{\sqrt{\delta}}}$ and $\pi / 2$.

Phase estimation is applied to the operator $U_D U_P$ in order to determine this angle, and to discriminate between the eigenvector 1 and the others. This is why only $\bigO{\frac{1}{\sqrt{\delta}}}$ calls to $U_D U_P$ are necessary, and where the quadratic speedup in the mixing time is obtained. Then, the phase of all eigenvectors with an eigenvalue different from 1 is flipped. This corresponds exactly to what we want to implement, that is, a reflection through $\ket{\pi}$, since only the eigenvector $\ket{\pi}$ is left unchanged.

The phase estimation circuit then consists in applying $(U_D U_P)^{2^s}$ for $s$ from $1$ to $\bigO{\log_2 \frac{1}{\sqrt{\delta}}}$, controlled by $\bigO{\log_2 \frac{1}{\sqrt{\delta}}}$ additional ancilla qubits (on which the estimated phase will be read afterwards). Note that~\cite{DBLP:journals/siamcomp/MagniezNRS11} performs multiples copies of this process in order to decide if the phase is $1$ with more fidelity.


\paragraph{Vertices of a Given Type.}
Between two walk steps, we can track the amplitudes of the vertices, since we know that marked and unmarked vertices in $\ket{\phi_i}$ have respectively equal amplitudes. However, in order to track the amplitudes inside the walk step, between two updates, we use a stronger assumption: that we are solving a subset-finding problem with a single solution. We define the ``type'' of a vertex as follows, depending on how far it is from being marked.

\AS{this definition and property should be extracted from \cite{DBLP:journals/qic/ChildsE05}, but I haven't found the precise statement. We can rename the "types"}

\begin{definition}[Classification of vertices]\label{def:classification}
A vertex $x = x_1, \ldots, x_t$ in the product Johnson graph is \emph{marked} if it contains a certain tuple $\vec{e}_1, \ldots, \vec{e}_t$, that is, if $\vec{e}_1 \in x_1, \ldots, \vec{e}_t \in x_t$. We partition the vertices $X$ into $2^t$ disjoint sets $X_0, \ldots, X_{2^t-1}$, depending on the subset of $\vec{e}_i$ that they contain, where $X_{2^t-1} = M$ is the marked set. The sets $X_i$ are the \emph{types} of vertices in the graph.
\end{definition}

%For each type of vertices, we can then consider the uniform superposition of its vertices: $\ket{t_j} = \sum_{x \in X_j} \ket{x} \ket{0} \ket{D(x)}$.
We can now remark that if the edges $(x,y)$, where $x \in X_i$, have all the same amplitude $t_i$ before applying $U_P$ (for all types $i$), then it remains the case afterwards.

\AS{with or without edges?}

\begin{lemma}
For a state of the form:
$$ \ket{\psi} = \sum_{0 \leq i \leq 2^t-1} \sum_{x \in X_i} \sum_{y} t_i \ket{x} \ket{y} \ket{D(x)} $$
then $U_P(\ket{\psi})$ has the same form (with different amplitudes).
\end{lemma}

\begin{proof} \AS{todo: details here}
All vertices of a given type have the same distribution of types among their neighbors, and $U_P$ treats all neighbors in the same way. Thus, the computation that leads to the amplitude of two vertices of a given type is the same. \qed
\end{proof}

\AS{so, basically, types are eigenvectors of $U_P$?}

Since $U_D$ only acts on the data structure, this property remains true of the whole update unitary $U_D U_P$.

Thus, inside a walk step, we can still control the individual amplitudes of vertices (since they are all the same for a given type). In particular, the only superpositions in input to $U_D$ are of this form.

\section{Perfect run of the walk, v2}
\subsection{Ideal setting: vertex-vertex encoding}
We consider a graph $G = (V,E)$ and for each $x \in V$, let $N_x$ bet the set of neighbors of $x$. For a vertex $x$, we denote by $D(x)$ the additional data associated to $x$. We define $\ket{\xh} = \ket{x}\ket{D(x)}$. Moreover, for a vertex $x$, let 
$\ket{p_x} = \frac{1}{\sqrt{|N_x|}} \sum_{y \in N_x} \ket{y}$ and 
$\ket{\widehat{p_x}} = \frac{1}{\sqrt{|N_x|}} \sum_{y \in N_x} \ket{\yh}$. We consider the space $A = span\{\ket{\xh}\ket{p_x}\}_{x \in V}$ and $B = span\{\ket{\pyh}\ket{y}\}_{y \in V}$.

Let $Ref_A$ and $Ref_B$ be respectively the reflexion over the space $A$ and the space $B$. 

\begin{proposition}[Fundamental MNRS quantum walk proposition] \label{Proposiiton:MNRS_Main}
	Let $W = Ref_B Ref_A$ and let $\ket{\psi_{\Unif}} = \frac{1}{\sqrt{|V|}} \sum_{x \in V} \ket{\xh}\ket{p_x}$. We have $
	\bra{\psi_{\Unif}} W\ket{\psi_{\Unif}} = 1$. 
	For any other eigenvector $\ket{\psi}$ of $W$, we have 
	$\bra{\psi} W\ket{\psi}  = e^{i\theta}$
	with $\theta  \in [2\sqrt{\delta},\pi/2]$.
\end{proposition}

A step of the quantum walk consists of constructing the unitary $W$, then we perform phase estimation wrt. $W$ in order to perform the reflexion over $\ket{\psi_{\Unif}}$. In order to construct $W$, we need to apply $Ref_A$ and $Ref_B$. In the query complexity model, we can perform $Ref_A$ without any quantum queries but we need queries to perform $Ref_B$. We will use the following construction for $$ Ref_B = \SWUP \circ Ref_A \circ \SWUP.$$
with $\SWUP \ket{\xh}\ket{y} = \ket{\yh}\ket{x}$. This $\SWUP$ (Swap-Update) operation can furthermore be decomposed into an update of the database followed by a register swap:

$$\ket{\xh}\ket{y} = \ket{x}\ket{D(x)}\ket{y} \xrightarrow{\UP_D} \ket{x}\ket{D(y)}\ket{y} \xrightarrow{\Swap} \ket{y}\ket{D(y)}\ket{x} = \ket{\yh}\ket{x}.$$
so $\SWUP = \Swap \circ \UP_D$. This $UP_D$ operator is what requires queries and, in the imperfect update case, which will be the source of errors when computing $W$. 

\subsection{Real time setting: Vertex-coin encoding}
The above construction is highly time inefficient. Indeed, the graphs we manipulate often have a very large $|V|$ and we can't afford even to spend $\log_2(|V|)$ for each update step. When $G$ is a $d$-regular graph, with $d << |V|$, we can use a vertex-coin encoding and manipulate only the edge register of size $\log_2(d)$. More precisely, we have a reversible encoding operation 

$$ O_{\Enc} \ket{\xh}\ket{y} = \ket{x}\ket{c_{x \rightarrow y}}.$$
where now, the second register is of size $\lceil \log_2(d) \rceil$. We want $\ket{c_{x \rightarrow y}} \bot \ket{c_{x\rightarrow y'}}$ for $y \neq y'$. Let $\ket{\psi_{\Unif}^{coin}} = \frac{1}{\sqrt{d}} \sum_{e} \ket{c}$ be the uniform set of coins. In the encoded, notice that $Ref_A$ corresponds to $I \otimes Ref_{\ket{\psi_{\Unif}^{coin}}}$, meaning that  
$$ Ref_A = O_{\Enc}^{-1} \circ \left(I \otimes Ref_{\ket{\psi_{\Unif}^{coin}}}\right) \circ O_{\Enc}.$$
Now, for the $\SWUP$ operation, we have to decompose again $\UP_D$ and $\Swap$ in the encoded space. First, we define $\UP'_D$ st. 
$$\ket{x}\ket{D(x)}\ket{e_{x \rightarrow y}} \xrightarrow{UP'_{D}} \ket{x}\ket{D(y)}\ket{e_{x \rightarrow y}}.$$

Moreover, we define $\Swap'$ st. 
$$\ket{x}\ket{e_{x \rightarrow y}} \xrightarrow{\Swap'} \ket{y}\ket{e_{y \rightarrow x}}.$$
and we define $\SWUP' = \Swap' \circ \UP'_D$ (we abuse notation here, by extending $\Swap'$ where we apply the identity to the middle register), so 

$$\SWUP' \ket{\xh}\ket{e_{x \rightarrow y}} = \ket{\yh}\ket{e_{y \rightarrow x}}.$$
and $\SWUP' = O_{\Enc} \circ \SWUP \circ O_{\Enc}^{-1}$. So we define 
\begin{align*}
	Ref'_A & = I \otimes Ref_{\ket{\psi_{\Unif}^{coin}}} = O_{\Enc} \circ Ref_A \circ O_{\Enc}^{-1} \\
	Ref'_B & = \SWUP' \circ Ref'_A \circ \SWUP' = O_{\Enc} \circ Ref_B \circ O_{\Enc}^{-1}  \\
	W' & = Ref'_B \circ Ref'_A 
\end{align*}
By putting everything together, we have $W' = O_{\Enc} \circ W \circ O_{\Enc}^{-1}$ so we can use Proposition \ref{Proposiiton:MNRS_Main} to have the spectral properties and perform phase estimation on $W'$. 

\subsection{Grover, quantum walks}
Consider two orthogonal vectors $\ket{\phi_B}$ and $\ket{\phi_G}$ and the $2$ dimensional subspace $\hh = span(\{\ket{\phi_B},\ket{\phi_G}\})$. Let $Rot_{\theta}$ be the $\theta$-rotation unitary in $\hh$ so
\begin{align*}
	Rot_\theta (\cos(\alpha)\ket{\phi_B} + \sin(\alpha)\ket{\psi_G}) = \cos(\alpha + \theta)\ket{\phi_B} + \sin(\alpha + \theta)\ket{\psi_G}
\end{align*}

For a fixed $\eps$, let
$$\ket{\phi_U} = \sqrt{1-\eps}\ket{\phi_B} + \sqrt{\eps}\ket{\phi_G} = \cos(\alpha)\ket{\phi_B} + \sin(\alpha)\ket{\phi_G},$$
so $\alpha = arccos(\sqrt{1-\eps})$. For a state $\ket{\psi} \in \hh$, let $Ref_{\ket{\psi}}$ be the reflexion over $\ket{\psi}$ in $\hh$ so 
\begin{align*}
	Ref_{\ket{\psi}} \ket{\psi}  = \ket{\psi} \quad \textrm{and} \quad
	Ref_{\ket{\psi}} \ket{\psi^\bot}  = - \ket{\psi^\bot} 
\end{align*}
where $\ket{\psi^\bot}$ is any state in $\hh$ orthogonal to $\ket{\psi}$\footnote{For a fixed $\ket{\psi}$, $\ket{\psi^\bot}$ is actually unique up to a global phase.}  We have
\begin{align}\label{Eq:RefToRot}
	Ref_{\ket{\psi_U}}Ref_{\ket{\psi_{B}}} = Rot_{2\alpha}.
\end{align}
We also have access to a checking oracle which performs the following operation:
\begin{align*}
	O_{check} \ket{\psi_{Bad}}\ket{0} & = \ket{\psi_{Bad}}\ket{0} \\
	O_{check} \ket{\psi_{Good}}\ket{0} & = \ket{\psi_{Good}}\ket{1}
\end{align*}

\begin{proposition}[Original Grover, known $\alpha$]\label{Proposition:GroverOriginal}
	Consider the following algorithm:
	\begin{enumerate}
		\item Start from $\ket{\psi_U}$. 
		\item Apply $R_{2\alpha} = Ref_{\ket{\psi_U}}Ref_{\ket{\psi_{B}}}$ $N$ times on $\ket{\psi_U}$ with $N = \lfloor\frac{\pi/2 - \alpha}{2\alpha}\rfloor$.
		\item Apply the checking oracle and measure the last qubit.
	\end{enumerate}
	This procedure measures $1$ wp. at least $1 - 2\alpha^2$ and the resulting state is $\ket{\psi_{Good}}$.
\end{proposition}
\begin{proof}
	Let us define $\gamma = \alpha + 2N\alpha$. We have 
	$$(Rot_{2\alpha})^n \ket{\psi_U} = \cos(\alpha + 2N\alpha)\ket{\phi_B} + \sin(\alpha + 2N\alpha)\ket{\phi_G} = \cos(\gamma)\ket{\phi_B} + \sin(\gamma)\ket{\phi_G}.$$
	Notice that we chose $N$ st. $\gamma \le \frac{\pi}{2} < \gamma + 2\alpha$ so $\frac{\pi}{2} - \gamma \in [0,2\alpha)$. After applying the checking oracle, we obtain the state 
	$$ \cos(\gamma)\ket{\phi_B}\ket{0} + \sin(\gamma)\ket{\phi_G}\ket{1}.$$
	Measuring the last qubit measures $1$ wp. $\sin^2(\gamma)$ and the resulting state in the first register is $\ket{\phi_G}$. In order to conclude, we compute 
	$$ \sin^2(\gamma) = \cos^2(\pi/2 - \gamma) \ge \cos^2(2\alpha) \ge 1 - 2\alpha^2.$$
\end{proof}		
\begin{proposition}[Starting from $\ket{\psi_B}$, known $\alpha$]\label{Proposition:GroverFromBad}
	Consider the following algorithm:
	\begin{enumerate}
		\item Start from $\ket{\psi_B}$. 
		\item Apply $R_{2\alpha} = Ref_{\ket{\psi_U}}Ref_{\ket{\psi_{B}}}$ $N'$ times on $\ket{\psi_B}$ with $N' = \lfloor\frac{\pi/2}{2\alpha}\rfloor$.
		\item Apply the checking oracle and measure the last qubit.
	\end{enumerate}
	This procedure measures $1$ wp. at least $1 - 2\alpha^2$ and the resulting state is $\ket{\psi_{Good}}$.
\end{proposition}
\begin{proof}
	The proof is essentially the same as the previous one. 
	Let $\gamma' =  2N\alpha$. We have 
	$$(Rot_{2\alpha})^n \ket{\psi_B} = \cos(2N\alpha)\ket{\phi_B} + \sin(2N\alpha)\ket{\phi_G} = \cos(\gamma')\ket{\phi_B} + \sin(\gamma')\ket{\phi_G}.$$
	Notice that we chose $N'$ st. $\gamma' \le \frac{\pi}{2} < \gamma' + 2\alpha$ so $\frac{\pi}{2} - \gamma' \in [0,2\alpha)$. After applying the checking oracle, we obtain the state 
	$$ \cos(\gamma')\ket{\phi_B}\ket{0} + \sin(\gamma')\ket{\phi_G}\ket{1}.$$
	Measuring the last qubit measures $1$ wp. $\sin^2(\gamma')$ and the resulting state in the first register is $\ket{\phi_G}$. In order to conclude, we compute 
	$$ \sin^2(\gamma') = \cos^2(\pi/2 - \gamma') \ge \cos^2(2\alpha) \ge 1 - 2\alpha^2.$$
\end{proof}		
\begin{proposition}[In place amplification of success probability]
	There is a quantum algorithm that, starting from $\ket{\psi_U}$, outputs $\ket{\psi_{Good}}$ wp. at least $1 - (2\alpha^2)^\kappa$ and that performs at most $\kappa N'$ calls to $R_{2\alpha} = Ref_{\ket{\psi_U}}Ref_{\ket{\psi_{B}}}$ with $N' = \lfloor\frac{\pi/2}{2\alpha}\rfloor$ and $\kappa$ measurements.
\end{proposition}
\begin{proof}
	We start from $\ket{\psi_U}$. First run the algorithm presented in Proposition~\ref{Proposition:GroverOriginal}. If you output $1$, stop and you have $\ket{\psi_{G}}$. Otherwise, you outputted $0$ and have the state $\ket{\psi_B}$. 
	
	In this case, run the algorithm presented in Proposition~\ref{Proposition:GroverFromBad}. If you output $1$, you have $\ket{\psi_G}$ and you stop. Otherwise, you have $\ket{\psi_B}$ again and you run this algorithm again. We allow at most $\kappa - 1$ repetitions of this second algorithm.
	
	Each algorithm succeeds wp. at least $1 - 2\alpha^2$ and we have $\kappa$ runs in total (1 time the first algortihm and at most $\kappa - 1$ times the second one), so the probability of failure is at most $(2\alpha^2)^\kappa$. Moreover, the second algorithm makes $N'$ calls to $R_{2\alpha}$ and the first one $N \le N'$ calls to $R_{2\alpha}$ so the total number of calls to $R_{2\alpha}$ is at most $\kappa N'$.
\end{proof}	









\COMMENT{
\section{Dealing with the double exponential size of $|V|$ and using coins in quantum walks + update}
\subsubsection{Coins.}
One problem when looking at quantum walks with real time is that the Johnson graph $J(n,r)$ has $|V| = \binom{n}{r}$  different vertices with $r = n^{\Omega(1)}$ so $\log(|V|) = n^{\Omega(1)}$. We usually have $n$ which is exponential so no matter the encoding of vertices, we need an exponential amount of qubits to store them. This makes it hard to justify that $U_P$ defined as
$$ U_P \left(\ket{x}_L\ket{0}_R\right) \rightarrow \frac{1}{\sqrt{|N_x|}} \ket{x}_L\sum_{y \in N_x} \ket{y}_R$$
can be efficiently computed, where $N_x$ is the set of neighbors of $x$. A way to deal with this problem is to use coins used in the quantum walk. We encode each vertex as a sorted list $x = (x_1,\dots,x_r)$ encoding a string $S \in \zo^n$ of weight $r$, st. $S_{i} = 1$ for $i \in L$ and $S_i = 0$ otherwise. A coin $c = (j,z)$ is a pair where $j \in [r]$ and $z \in [n-r]$ a new index. From a vertex $X = (x_1,\dots,x_r)$, we define the vertex $x+c$ where we remove $x_j$ from $x$ and then add the $z^{th}$ from the set $[n]\backslash X$, which we call by abuse of notation $z$. So we have 
$$ x + c = \left(x_1,\dots,x_{j-1},x_{j+1},\dots,z,\dots,x_r\right).$$
Since the list in vertices is sorted, $z$ can be at a different position than $x_j$ was. Let $\cc$ be the set of possible coins. Instead of encoding $\ket{x}\ket{y}$, we encode $\ket{x}\ket{c : x+c = y}$. Since $\log(|C|)$ is logarithmic in $n$, $U_P$ can be  done efficiently. We are interested in the following operations:
\begin{align*}
\ket{x}\ket{0}\ket{D(x)} & \xrightarrow{U_P} \frac{1}{\sqrt{|C|}} \sum_{c \in \cc} \ket{x}\ket{c}\ket{D(x)} \\
& \xrightarrow{U_D} \frac{1}{\sqrt{|C|}} \sum_{c \in \cc} \ket{x}\ket{c}\ket{D(x + c)} \\
& \xrightarrow{U'} \frac{1}{\sqrt{|C|}} \sum_{y \in N_x} \ket{y}\ket{c' : y + c' = x}\ket{D(y)} \\
\end{align*}
The unitary $U' : \ket{x}\ket{c} \rightarrow  \ket{y = x+c}\ket{c': y + c' = x}$ can be a bit tricky but it should be doable with a proper quantum data structure but this shows we need $QRA(Q)M$ already at this step and not only in $U_D$. Then, after applying $U' \circ U_D \circ U_P$, we check that the middle register is a superposition of all the coins. This operation can be done efficiently. Similarly as in usual quantum walks, we should be able to show that this is satisfied only if we start from the state $\ket{\psi} = \frac{1}{\sqrt{|V|}}\sum_{x \in V}\ket{x}\ket{0}\ket{D(x)}$ so we can use this procedure to perform a reflexion of $\ket{\psi}$ using phase estimation. 
\subsubsection{Update.}
In practice, we have $\wU_D$ st. $\wU_D \ket{x}\ket{c}\ket{D(x)} = \ket{x}\ket{c}\ket{D(x+c)}$ for an $(1 - \mu)$ fraction of $(x,c)$.
Let us write $\ket{\psi_{Good}} = \frac{1}{\sqrt{|V_{Good}||\cc|}}\sum_{x \in V_{Good},c}\ket{x}\ket{c}\ket{D(x)}$ and $\ket{\psi_{Bad}} = \frac{1}{\sqrt{|V_{Bad}||\cc|}}\sum_{x \in V_{Bad},c}\ket{x}\ket{c}\ket{D(x)}$ (the good and bad vertices and the marked and unmarked vertices). What we need to show is that $\wU_D$ behaves very closely to $U_D$ on the subspace $\{\ket{\psi_{Bad}},\ket{\psi_{Good}}\}$.

When comparing $\wU_D \ket{\psi_{Bad}}$ with $U \ket{\psi_{Bad}}$, the difference is a function of $\frac{\mu |V| |\cc|}{|V_{Bad}| |\cc|} = \frac{\mu}{1-\eps}$ where $\eps$ is the fraction of marked vertices. We don't specify what distance function to take but for any reasonable function, it will be a function of $\frac{\mu}{1-\eps}$. Similarly, when comparing $\wU_D \ket{\psi_{Good}}$ with $U \ket{\psi_{Good}}$, the distance between these $2$ states is in the worst case $\frac{\mu}{\eps}$ where $\mu \ll \eps$. We perform $\frac{\sqrt{r}}{\sqrt{\eps}}$ steps of the random walk so in the end, we would like $\mu \ll \sqrt{\frac{r}{\eps^3}}$ for the whole error not to blow up (maybe there are some squares depending on the distance function we use but if we have a tiny $\mu$, we can deal with this).

\subsubsection{More formally}

\begin{proposition}[Simplified case]
	Let $U$ be a unitary  on $\hh = \mathbb{C}^{2^n}$ and let $\hh'$ be a subspace of $\hh$. Assume  that for any quantum state $\ket{\phi} \in \hh', \ U \ket{\phi} \in \hh'$. Moreover, consider a unitary $\wU$ st. for any quantum state $\ket{\phi} \in \hh'$, 
	\begin{align}\label{Eq:1}
		|\bra{\phi} U^\dagger \wU \ket{\phi}| \ge \sqrt{1-\mu}.
	\end{align}
	For any $\ket{\phi} \in \hh'$, for any $N \in \mathbb{N}$, there exists $\ket{Z_N}$ st.  
	\begin{align*}
		\wU^{N} \ket{\phi} = \alpha_N U^{N}\ket{\phi} + \beta_N \ket{Z_N}
	\end{align*}
with $1 \ge |\alpha_N| \ge \left(\sqrt{1 - \mu}\right)^N$ and $|\beta_N| \le N \sqrt{\mu}$.  $\ket{Z_N}$ is a normalized quantum state in $\hh$ not necessarily orthogonal to $\ket{\phi}$.
\end{proposition}
\begin{proof}
	We prove this by induction. It's clearly true for $N = 0$. Assume we have for a fixed value $N$, so we write 
	\begin{align*}
		\wU^{N} \ket{\phi} = \alpha_N U^{N}\ket{\phi} + \beta_N \ket{Z_N}
	\end{align*}
which satisfy the above. Let $\ket{\phi_N} = U^N \ket{\phi}$. From Equation \ref{Eq:1}, we have 
$$ \wU \ket{\phi_N} = \alpha U\ket{\phi_N} + \beta \ket{Y}.$$
with $\ket{Y} \bot \ U\ket{\phi_N}$ and $1 \ge |\alpha| \ge \sqrt{1- \mu}$ which gives $|\beta| \le \sqrt{\mu}$. Plugging this in the above, we have 
\begin{align*}
	\wU(\ket{\phi_{N}}) & = \alpha_N\left(\alpha \ket{\phi_{N+1}} + \beta \ket{Y}\right) + \beta_N \wU \ket{Z_N} \\
	& = \alpha \alpha_N \ket{\phi_{N+1}} + \alpha_N \beta \ket{Y} + \beta_N \wU\ket{Z_N}
\end{align*}
We clearly have $1 \ge |\alpha \alpha_N| \le \left(\sqrt{1-\mu}\right)^{N+1}$. Moreover, the  norm of  $\alpha_N \beta \ket{Y} + \beta_N \wU\ket{Z_N}$ is at most $|\alpha_N \beta| + |\beta_N| \le (N+1)\sqrt{\mu}$, so we can write 
$$\alpha_N \beta \ket{Y} + \beta_N \wU\ket{Z_N} = \beta_{N+1}\ket{Z_{N+1}}$$
for a normalized $\ket{Z_{N+1}}$ and $|\beta_{N+1}| \le (N+1)\sqrt{\mu}$ which finished the proof. 
\end{proof}
\begin{corollary}
	For any $\ket{\phi} \in \hh'$, for any $N \in \mathbb{N}$ we have 
	$$|\bra{\phi} \left(U^N\right)^\dagger \wU ^N\ket{\phi}| \ge |\alpha_N| - |\beta_N| \ge 1 - \left(\sqrt{1-\mu}\right)^N - N\sqrt{\mu}.$$
\end{corollary}

\paragraph{Real case.}
In the real case, we don't just perform $N$ calls to the update function but we perform in between other operations. Since these other operations stabilize $\hh'$, we can use the same proof as above for this more general case and obtain the same result. 

\subsection{A walk with Imperfect Updates}

%\newcommand{\pbadedges}{p_{\mathsf{bad}}}

We are now replacing the perfect data update $U_D$ with an imperfect update $U_D'$. $U_D'$ still works ``most of the time'', in a way that we have to quantify. First of all, we say that an edge $(x,y)$ is bad if $U_D'$ does not map $\ket{x} \ket{y} \ket{D(x)}$ to $\ket{x} \ket{y} \ket{D(y)}$ as expected (whatever the reason). We define a notion of ``$p$-bad vertices'', which are vertices with too many bad edges.

\begin{definition}
$x$ is a $p$-bad vertex iff there exists a type of vertices such that the proportion of bad edges $(x,y)$ among neighbors $y$ of this type exceeds $p$.
\end{definition}

We expect the bad vertices to be clustered, since at many places in the graph, changing a single element in the vertex will not change its bad status.

\begin{assumption}
There exists an exponentially small parameter $p'$ such that, for any type, the proportion of $p$-bad vertices is smaller than $p'$.
\end{assumption}

We now show that, with this assumption, we can run the walk with $U_D'$, and this does not disrupt too much the final state. More precisely:

\begin{lemma}\label{lemma:bound-bad}
Let $\ket{\psi}$ the state before any update unitary $U_D$, then:
$$ \| U_D \ket{\psi}- U_D' \ket{\psi} \| \leq p' + (1-p')p \enspace. $$
\end{lemma}

\begin{proof}
We write:
$$ \ket{\psi} = \sum_{0 \leq i \leq 2^t-1} \sum_{x \in X_i} \sum_{y} t_i \ket{x} \ket{y} \ket{D(x)} \enspace. $$
For each vertex $x$, there exists bad edges $(x,y)$. However the proportion of bad edges is quite small; unless the vertex is $p$-bad, in which case it's the proportion of such vertices themselves which is also small. More precisely, we have that:
\[ \forall x \in X_i, \text{if $x$ is not $p$-bad}, \| U_D( \sum_y \ket{x} \ket{y} \ket{D(x)} ) - U_D'(\sum_y \ket{x} \ket{y} \ket{D(x)})  \|^2 \leq p' \enspace.  \]
That's because the superposition over all edges $(x,y)$ is uniform \AS{check that}

Next:
\[ \| U_D \ket{\psi}- U_D' \ket{\psi} \|^2 = \sum_i t_i^2 \| \sum_{x \in X_i} U_D( \sum_{y} \ket{x} \ket{y} \ket{D(x)})  -  U_D'( \sum_{y} \ket{x} \ket{y} \ket{D(x)}) \|^2 \leq p' + (1-p')p \enspace. \]

\end{proof}


\begin{theorem}\label{theorem:imperfect-qw}
Assume that $p' + (1-p')p < \epsilon \delta$, then running the quantum walk with $U_D'$ (instead of $U_D$) leads to a marked vertex with constant probability.
\end{theorem}

\begin{proof}[Proof of~\autoref{theorem:imperfect-qw}]
Each time we apply $U_D'$ instead of $U_D$, the state $\ket{\psi_t'}$ of the walk at step $t$ moves away from its ideal state $\ket{\psi_t}$, which is the state that we would have obtained with a perfect $U_D$. More precisely, we define: $U_D' \ket{\psi_t} = \ket{\psi_{t+1}^{\mathrm{good}}} + \ket{\psi_{t+1}^{\mathrm{bad}}}$, where $\ket{\psi_{t+1}^{\mathrm{bad}}}$ is the error term introduced due to the handling of ``bad'' edges. The total distance between $\ket{\psi_t'}$ and $\ket{\psi_t}$ can then be bounded via a ``hybrid argument'' as in~\cite{DBLP:journals/siamcomp/BennettBBV97,DBLP:journals/siamcomp/Ambainis07}:
%\begin{lemma}[\cite{DBLP:journals/siamcomp/Ambainis07}, Lemma 5]\label{lemma:hybrid}
\begin{equation}\label{eq:hybrid}
\| \ket{\psi_t} - \ket{\psi_t'} \| \leq 2 \sum_{i=1}^t \| \ket{\psi_i^{\mathrm{bad}}} \|
\end{equation}
Then the norm of $\ket{\psi_i^{\mathrm{bad}}}$ is bounded by~\autoref{lemma:bound-bad}. Since the imperfect update is applied $\bigO{ \frac{1}{\sqrt{\epsilon \delta}}}$ times, it suffices to have: $C \sqrt{p' + (1-p')p} \frac{1}{\sqrt{\epsilon \delta}} < 1$ for some constant $C$ in order to ensure that the norm of the difference between the final state in the ``perfect'' walk and the real result is less than a small constant. Then, the variation distance between the probability distributions on outcomes of both algorithms is less than a constant as well~\cite{bernstein1997quantum}, and the theorem follows. 
\qed
\end{proof}



%As there are $2^t$ types, and this is a constant, the amplitude of a given basis state will remain negligibly low. This helps us to show that the amplitude on ``bad'' edges remains low, after which we will apply Equation (\ref{eq:hybrid}).
%
%%As bad edges are uniformly distributed among good and bad states, and there are relatively few of them, it is impossible that a massive amplitude suddenly moves to the ``bad'' part $\ket{\psi_i^{\mathrm{bad}}}$ of the current state. Thus
%
%Let $\ket{\psi_{i-1}}$ be the perfect current state before applying the imperfect data structure update. By Lemma~\ref{lemma:equalampl2}, $\ket{\psi_{i-1}}$ is the sum of uniform superposition over types of vertices:
%$$ \ket{\psi_{i-1}} = \alpha_0 \sum_{(x,y), x \in X_1} \ket{x y} + \ldots + \alpha_{2^t -1} \sum_{(x,y), x \in X_{2^t-1}} \ket{x y}  $$
%where $\alpha_i \leq \frac{1}{\sqrt{|X_i|}}$. In particular, at the beginning of the computation, the amplitude is uniformly distributed over all edges, and at the end, it falls uniformly on all edges $(x,y)$ where $x \in M$. Next, we sum the errors over all these subcomponents:
%\begin{equation}\label{eq:psibad}
%\| \ket{\psi_i^{\mathrm{bad}}} \|^2 \leq \sum_{1 \leq i \leq 2^t} \frac{1}{|X_i|} | \{x \in X_i, (x,y) \text{ bad} \}| = \sum_{1 \leq i \leq 2^t} \prob[x \in X_i, y \text{ random }]{(x,y) \text{ bad}}
%\end{equation}



\subsection{Errors in the Setup}

In Theorem~\ref{theorem:imperfect-qw}, we assumed that the initial state $\ket{\pi}$ obtained from the quantum walk setup was \emph{perfect}, in the sense that each state had its correct data structure. But, similarly to the errors in the update, the setup need not be a perfect unitary. In fact, in our case, many vertices are ``bad'', and the \texttt{Setup} procedure creates invalid data structures for them.

Let $\ket{\pi}$ be the \emph{perfect} setup state and $\ket{\pi}'$ the imperfect one. Let $W$ be the unitary that realizes the whole walk (with an imperfect update). Then we have:
$$ \|  \ket{\pi} - \ket{\pi}' \| = \|  W \ket{\pi} -  W\ket{\pi}' \| \enspace. $$
Thus, the final state of the walk deviates from the expected $(W \ket{\pi})$ only as much as the initial state. By combining this with Theorem~\ref{theorem:imperfect-qw}, we obtain:

\begin{corollary}[Imperfect quantum walk]
Consider a walk on a Johnson graph with imperfect setup and updates, and a perfect checking unitary. Assume that the probability of being a ``bad'' node in the setup is  a small constant. Assume that $p_{\mathrm{bad}}$ is $o(\delta \epsilon)$. Then the ``imperfect'' quantum walk returns a marked vertex with constant probability.
\end{corollary}


}
%In the quantum walk algorithms that we studied in this paper, the checking time is negligible, and the optimization leads to a setup time $\mathsf{S}$ that is equal to the walk time $\frac{1}{\sqrt{\epsilon} \sqrt{\delta}} \mathsf{U}$. This makes possible to describe the setup as a \emph{sequence of updates}, which also contains $\frac{1}{\sqrt{\epsilon} \sqrt{\delta}}$

==> files/ideal-walk.tex <==
% !TeX root = ../collision-walk.tex



\section{Quantum walks}

\AS{j'ai juste déplacé ici du texte qu'on va peut-être réutiliser}

In this section, we give a generic analysis on quantum walks on product Johnson graphs, which is a specialization of~\cite{DBLP:journals/siamcomp/MagniezNRS11} and Section 4.1 in~\cite{DBLP:phd/basesearch/Jeffery14}. An analysis of quantum walks for subset-finding is also given in~\cite{DBLP:journals/qic/ChildsE05}, which generalizes the study of~\cite{DBLP:journals/siamcomp/Ambainis07}. Though more generic frameworks exist, none of them have seen cryptographic applications so far.



The quantum walk algorithm is analogous to a classical random walk on a regular, undirected graph. In our case, this graph is a \emph{product Johnson graph}.

\begin{definition}[Johnson graph]
Let $X$ be a set of size $N$. The Johnson graph $J(X, R)$ is an undirected graph whose vertices are the subsets of $X$ containing $R$ elements, with an edge between two vertices $u$ and $u'$ iff $|u\cap u'|=R-1$. In other words, $u$ is adjacent to $u'$ if $u'$ can be obtained from $u$ by removing an element and adding a new element in its place.
\end{definition}

\begin{definition}[Product of graphs]
	Let $G_1=(\mathcal{V}_1,\mathcal{E}_1)$ and $G_2=(\mathcal{V}_2,\mathcal{E}_2)$ be two graphs, their product $G_1\times G_2$ is the graph $G=(\mathcal{V},\mathcal{E})$ where: 
	\begin{enumerate}
		\item $\mathcal{V}=\mathcal{V}_1\times \mathcal{V}_2$, i.e. $\mathcal{V}=\{v_1v_2|v_1\in\mathcal{V}_1,v_2\in\mathcal{V}_2\} $
		\item $\mathcal{E}=\{(u_1u_2,v_1v_2)|(u_1=v_1 \wedge (u_2,v_2)\in \mathcal{E}_2) \vee ((u_1,v_1)\in \mathcal{E}_1 \wedge u_2=v_2 )\}$
	\end{enumerate}
	
\end{definition}

\begin{definition}[Product Johnson graph]
Let $X_1, \ldots, X_t$ be sets of size $N_1, \ldots, N_t$. The product Johnson graph $G = J(X_1, \ldots, X_t ; R_1, \ldots, R_t)$ is the product graph $J(X_1,R_1)\times \ldots \times J(X_t,R_t)$.

We identify a vertex $u = (u_1, \ldots, u_t)$ with a tuple of subsets of $X_1 \times \ldots \times X_t$.
\end{definition}



\section{Perfect run of the walk, v2}
\subsection{Ideal setting: vertex-vertex encoding}
We consider a graph $G = (V,E)$ which is $d$-regular and for each $x \in V$, let $N_x$ be the set of neighbors of $x$. For a vertex $x$, we denote by $D(x)$ the additional data associated to $x$. We define $\ket{\xh} = \ket{x}\ket{D(x)}$. Moreover, for a vertex $x$, let 
$\ket{p_x} = \frac{1}{\sqrt{|N_x|}} \sum_{y \in N_x} \ket{y}$ and 
$\ket{\widehat{p_x}} = \frac{1}{\sqrt{|N_x|}} \sum_{y \in N_x} \ket{\yh}$. We consider the space $A = span\{\ket{\xh}\ket{p_x}\}_{x \in V}$ and $B = span\{\ket{\pyh}\ket{y}\}_{y \in V}$.

Let $Ref_A$ and $Ref_B$ be respectively the reflexion over the space $A$ and the space $B$. 

\begin{proposition}[Fundamental MNRS quantum walk proposition] \label{Proposiiton:MNRS_Main}
	Let $W = Ref_B Ref_A$ and let $\ket{\psi_{\Unif}} = \frac{1}{\sqrt{|V|}} \sum_{x \in V} \ket{\xh}\ket{p_x}$. We have $
	\bra{\psi_{\Unif}} W\ket{\psi_{\Unif}} = 1$. 
	For any other eigenvector $\ket{\psi}$ of $W$, we have 
	$\bra{\psi} W\ket{\psi}  = e^{i\theta}$
	with $\theta  \in [2\sqrt{\delta},\pi/2]$.
\end{proposition}

A step of the quantum walk consists of constructing the unitary $W$, then we perform phase estimation wrt $W$ in order to perform the reflexion over $\ket{\psi_{\Unif}}$. In order to construct $W$, we need to apply $Ref_A$ and $Ref_B$. In the query complexity model, we can perform $Ref_A$ without any quantum queries but we need queries to perform $Ref_B$. We will use the following construction for $$ Ref_B = \SWUP \circ Ref_A \circ \SWUP.$$
with $\SWUP \ket{\xh}\ket{y} = \ket{\yh}\ket{x}$. This $\SWUP$ (Swap-Update) operation can furthermore be decomposed into an update of the database followed by a register swap:

$$\ket{\xh}\ket{y} = \ket{x}\ket{D(x)}\ket{y} \xrightarrow{\UP_D} \ket{x}\ket{D(y)}\ket{y} \xrightarrow{\Swap} \ket{y}\ket{D(y)}\ket{x} = \ket{\yh}\ket{x}.$$
so $\SWUP = \Swap \circ \UP_D$. This $UP_D$ operator is what requires queries and, in the imperfect update case, which will be the source of errors when computing $W$. 

\subsection{Real time setting: Vertex-coin encoding}
The above construction is highly time inefficient. Indeed, the graphs we manipulate often have a very large $|V|$ and we can't afford even to spend $\log_2(|V|)$ for each update step. When $G$ is a $d$-regular graph, with $d \ll |V|$, we can use a vertex-coin encoding and manipulate only the edge register of size $\log_2(d)$. More precisely, we have a reversible encoding operation 

$$ O_{\Enc} \ket{\xh}\ket{y} = \ket{\xh}\ket{c_{x \rightarrow y}}.$$
where now, the second register is of size $\lceil \log_2(d) \rceil$. We want $\ket{c_{x \rightarrow y}} \bot \ket{c_{x\rightarrow y'}}$ for $y \neq y'$. Let $\ket{\psi_{\Unif}^{coin}} = \frac{1}{\sqrt{d}} \sum_{c} \ket{c}$ be the uniform set of coins. In the vertex-coin encoding, notice that $Ref_A$ corresponds to $I \otimes Ref_{\ket{\psi_{\Unif}^{coin}}}$, meaning that  
$$ Ref_A = O_{\Enc}^{-1} \circ \left(I \otimes Ref_{\ket{\psi_{\Unif}^{coin}}}\right) \circ O_{\Enc}.$$
Now, for the $\SWUP$ operation, we have to decompose again $\UP_D$ and $\Swap$ in the encoded space. First, we define $\UP'_D$ st. 
$$\ket{x}\ket{D(x)}\ket{c_{x \rightarrow y}} \xrightarrow{UP'_{D}} \ket{x}\ket{D(y)}\ket{c_{x \rightarrow y}}.$$

Moreover, we define $\Swap'$ st. 
$$\ket{x}\ket{c_{x \rightarrow y}} \xrightarrow{\Swap'} \ket{y}\ket{c_{y \rightarrow x}}.$$
and we define $\SWUP' = \Swap' \circ \UP'_D$ (we abuse notation here, by extending $\Swap'$ where we apply the identity to the middle register), so 

$$\SWUP' \ket{\xh}\ket{c_{x \rightarrow y}} = \ket{\yh}\ket{c_{y \rightarrow x}}.$$
and $\SWUP' = O_{\Enc} \circ \SWUP \circ O_{\Enc}^{-1}$. So we define 
\begin{align*}
	Ref'_A & = I \otimes Ref_{\ket{\psi_{\Unif}^{coin}}} = O_{\Enc} \circ Ref_A \circ O_{\Enc}^{-1} \\
	Ref'_B & = \SWUP' \circ Ref'_A \circ \SWUP' = O_{\Enc} \circ Ref_B \circ O_{\Enc}^{-1}  \\
	W' & = Ref'_B \circ Ref'_A 
\end{align*}
By putting everything together, we have $W' = O_{\Enc} \circ W \circ O_{\Enc}^{-1}$ so we can use Proposition \ref{Proposiiton:MNRS_Main} to have the spectral properties and perform phase estimation on $W'$. 



\section{Dealing with the double exponential size of $|V|$ and using coins in quantum walks + update}
\subsubsection{Coins.}
One problem when looking at quantum walks with real time is that the Johnson graph $J(n,r)$ has $|V| = \binom{n}{r}$  different vertices with $r = n^{\Omega(1)}$ so $\log(|V|) = n^{\Omega(1)}$. We usually have $n$ which is exponential so no matter the encoding of vertices, we need an exponential amount of qubits to store them. This makes it hard to justify that $U_P$ defined as
$$ U_P \left(\ket{x}_L\ket{0}_R\right) \rightarrow \frac{1}{\sqrt{|N_x|}} \ket{x}_L\sum_{y \in N_x} \ket{y}_R$$
can be efficiently computed, where $N_x$ is the set of neighbors of $x$. A way to deal with this problem is to use coins used in the quantum walk. We encode each vertex as a sorted list $x = (x_1,\dots,x_r)$ encoding a string $S \in \zo^n$ of weight $r$, st. $S_{i} = 1$ for $i \in L$ and $S_i = 0$ otherwise. A coin $c = (j,z)$ is a pair where $j \in [r]$ and $z \in [n-r]$ a new index. From a vertex $X = (x_1,\dots,x_r)$, we define the vertex $x+c$ where we remove $x_j$ from $x$ and then add the $z^{th}$ from the set $[n]\backslash X$, which we call by abuse of notation $z$. So we have 
$$ x + c = \left(x_1,\dots,x_{j-1},x_{j+1},\dots,z,\dots,x_r\right).$$
Since the list in vertices is sorted, $z$ can be at a different position than $x_j$ was. Let $\cc$ be the set of possible coins. Instead of encoding $\ket{x}\ket{y}$, we encode $\ket{x}\ket{c : x+c = y}$. Since $\log(|C|)$ is logarithmic in $n$, $U_P$ can be  done efficiently. We are interested in the following operations:
\begin{align*}
\ket{x}\ket{0}\ket{D(x)} & \xrightarrow{U_P} \frac{1}{\sqrt{|C|}} \sum_{c \in \cc} \ket{x}\ket{c}\ket{D(x)} \\
& \xrightarrow{U_D} \frac{1}{\sqrt{|C|}} \sum_{c \in \cc} \ket{x}\ket{c}\ket{D(x + c)} \\
& \xrightarrow{U'} \frac{1}{\sqrt{|C|}} \sum_{y \in N_x} \ket{y}\ket{c' : y + c' = x}\ket{D(y)} \\
\end{align*}
The unitary $U' : \ket{x}\ket{c} \rightarrow  \ket{y = x+c}\ket{c': y + c' = x}$ can be a bit tricky but it should be doable with a proper quantum data structure but this shows we need $QRA(Q)M$ already at this step and not only in $U_D$. Then, after applying $U' \circ U_D \circ U_P$, we check that the middle register is a superposition of all the coins. This operation can be done efficiently. Similarly as in usual quantum walks, we should be able to show that this is satisfied only if we start from the state $\ket{\psi} = \frac{1}{\sqrt{|V|}}\sum_{x \in V}\ket{x}\ket{0}\ket{D(x)}$ so we can use this procedure to perform a reflexion of $\ket{\psi}$ using phase estimation. 
\subsubsection{Update.}
In practice, we have $\wU_D$ st. $\wU_D \ket{x}\ket{c}\ket{D(x)} = \ket{x}\ket{c}\ket{D(x+c)}$ for an $(1 - \mu)$ fraction of $(x,c)$.
Let us write $\ket{\psi_{Good}} = \frac{1}{\sqrt{|V_{Good}||\cc|}}\sum_{x \in V_{Good},c}\ket{x}\ket{c}\ket{D(x)}$ and $\ket{\psi_{Bad}} = \frac{1}{\sqrt{|V_{Bad}||\cc|}}\sum_{x \in V_{Bad},c}\ket{x}\ket{c}\ket{D(x)}$ (the good and bad vertices and the marked and unmarked vertices). What we need to show is that $\wU_D$ behaves very closely to $U_D$ on the subspace $\{\ket{\psi_{Bad}},\ket{\psi_{Good}}\}$.

When comparing $\wU_D \ket{\psi_{Bad}}$ with $U \ket{\psi_{Bad}}$, the difference is a function of $\frac{\mu |V| |\cc|}{|V_{Bad}| |\cc|} = \frac{\mu}{1-\eps}$ where $\eps$ is the fraction of marked vertices. We don't specify what distance function to take but for any reasonable function, it will be a function of $\frac{\mu}{1-\eps}$. Similarly, when comparing $\wU_D \ket{\psi_{Good}}$ with $U \ket{\psi_{Good}}$, the distance between these $2$ states is in the worst case $\frac{\mu}{\eps}$ where $\mu \ll \eps$. We perform $\frac{\sqrt{r}}{\sqrt{\eps}}$ steps of the random walk so in the end, we would like $\mu \ll \sqrt{\frac{r}{\eps^3}}$ for the whole error not to blow up (maybe there are some squares depending on the distance function we use but if we have a tiny $\mu$, we can deal with this).

\subsubsection{More formally}

\begin{proposition}[Simplified case]
	Let $U$ be a unitary  on $\hh = \mathbb{C}^{2^n}$ and let $\hh'$ be a subspace of $\hh$. Assume  that for any quantum state $\ket{\phi} \in \hh', \ U \ket{\phi} \in \hh'$. Moreover, consider a unitary $\wU$ st. for any quantum state $\ket{\phi} \in \hh'$, 
	\begin{align}\label{Eq:1}
		|\bra{\phi} U^\dagger \wU \ket{\phi}| \ge \sqrt{1-\mu}.
	\end{align}
	For any $\ket{\phi} \in \hh'$, for any $N \in \mathbb{N}$, there exists $\ket{Z_N}$ st.  
	\begin{align*}
		\wU^{N} \ket{\phi} = \alpha_N U^{N}\ket{\phi} + \beta_N \ket{Z_N}
	\end{align*}
with $1 \ge |\alpha_N| \ge \left(\sqrt{1 - \mu}\right)^N$ and $|\beta_N| \le N \sqrt{\mu}$.  $\ket{Z_N}$ is a normalized quantum state in $\hh$ not necessarily orthogonal to $\ket{\phi}$.
\end{proposition}
\begin{proof}
	We prove this by induction. It's clearly true for $N = 0$. Assume we have for a fixed value $N$, so we write 
	\begin{align*}
		\wU^{N} \ket{\phi} = \alpha_N U^{N}\ket{\phi} + \beta_N \ket{Z_N}
	\end{align*}
which satisfy the above. Let $\ket{\phi_N} = U^N \ket{\phi}$. From Equation \ref{Eq:1}, we have 
$$ \wU \ket{\phi_N} = \alpha U\ket{\phi_N} + \beta \ket{Y}.$$
with $\ket{Y} \bot \ U\ket{\phi_N}$ and $1 \ge |\alpha| \ge \sqrt{1- \mu}$ which gives $|\beta| \le \sqrt{\mu}$. Plugging this in the above, we have 
\begin{align*}
	\wU(\ket{\phi_{N}}) & = \alpha_N\left(\alpha \ket{\phi_{N+1}} + \beta \ket{Y}\right) + \beta_N \wU \ket{Z_N} \\
	& = \alpha \alpha_N \ket{\phi_{N+1}} + \alpha_N \beta \ket{Y} + \beta_N \wU\ket{Z_N}
\end{align*}
We clearly have $1 \ge |\alpha \alpha_N| \le \left(\sqrt{1-\mu}\right)^{N+1}$. Moreover, the  norm of  $\alpha_N \beta \ket{Y} + \beta_N \wU\ket{Z_N}$ is at most $|\alpha_N \beta| + |\beta_N| \le (N+1)\sqrt{\mu}$, so we can write 
$$\alpha_N \beta \ket{Y} + \beta_N \wU\ket{Z_N} = \beta_{N+1}\ket{Z_{N+1}}$$
for a normalized $\ket{Z_{N+1}}$ and $|\beta_{N+1}| \le (N+1)\sqrt{\mu}$ which finished the proof. 
\end{proof}
\begin{corollary}
	For any $\ket{\phi} \in \hh'$, for any $N \in \mathbb{N}$ we have 
	$$|\bra{\phi} \left(U^N\right)^\dagger \wU ^N\ket{\phi}| \ge |\alpha_N| - |\beta_N| \ge 1 - \left(\sqrt{1-\mu}\right)^N - N\sqrt{\mu}.$$
\end{corollary}

\paragraph{Real case.}
In the real case, we don't just perform $N$ calls to the update function but we perform in between other operations. Since these other operations stabilize $\hh'$, we can use the same proof as above for this more general case and obtain the same result. 

